TAEN: A Model-Constrained Tikhonov Autoencoder Network for Forward and Inverse Problems

Efficient real-time solvers for forward and inverse problems are essential in engineering and science applications. Machine learning surrogate models have emerged as promising alternatives to traditional methods, offering substantially reduced computational time. Nevertheless, these models typically demand extensive training datasets to achieve robust generalization across diverse scenarios. While physics-based approaches can partially mitigate this data dependency and ensure physics-interpretable solutions, addressing scarce data regimes remains a challenge. Both purely data-driven and physics-based machine learning approaches demonstrate severe overfitting issues when trained with insufficient data. We propose a novel Tikhonov autoencoder model-constrained framework, called TAE, capable of learning both forward and inverse surrogate models using a single arbitrary observation sample. We develop comprehensive theoretical foundations including forward and inverse inference error bounds for the proposed approach for linear cases. For comparative analysis, we derive equivalent formulations for pure data-driven and model-constrained approach counterparts. At the heart of our approach is a data randomization strategy, which functions as a generative mechanism for exploring the training data space, enabling effective training of both forward and inverse surrogate models from a single observation, while regularizing the learning process. We validate our approach through extensive numerical experiments on two challenging inverse problems: 2D heat conductivity inversion and initial condition reconstruction for time-dependent 2D Navier-Stokes equations. Results demonstrate that TAE achieves accuracy comparable to traditional Tikhonov solvers and numerical forward solvers for both inverse and forward problems, respectively, while delivering orders of magnitude computational speedups.

==> Figs/mcDecoder_architecture.tex <==
\def\layersep{1.2cm}
\def\nodeinlayersep{0.8cm}


\begin{figure}[H]
\centering
\begin{tikzpicture}[
    node distance=\layersep,
    edge/.style={-stealth,shorten >=1pt, draw=black!50,thin},
    neuron/.style={circle,fill=black!25,minimum size=10pt,inner sep=0pt},
    operator/.style={rectangle,fill=green!,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, inner sep=0pt, rounded corners},
    input neuron/.style={neuron, fill=green!50,minimum size=16pt},
    output neuron/.style={neuron, fill=green!50,minimum size=12pt},
    hidden neuron/.style={neuron, fill=blue!50},
    Forward map/.style={operator, fill=red!50},
    annot/.style={text width=4em, text centered},
    every node/.style={scale=1.0},
    node1/.style={scale=2.0}
]
    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
        {\ifnum \y=3
            \node (I-\name) at (0,-\nodeinlayersep * \y - \nodeinlayersep * 0.5) {$\vdots$};
            % \node[input neuron] (I-\name) at (0,-\y-0.4) {$y_{\y}$};
        \else
            \ifnum \y=4
                \node[input neuron] (I-\name) at (0,-\nodeinlayersep * \y - \nodeinlayersep * 0.5) {$u_{m}$};
            \else
                \node[input neuron] (I-\name) at (0,-\nodeinlayersep *\y - \nodeinlayersep * 0.5 ) {$u_{\y}$};
            \fi
        \fi}
        
    % Draw the output layer node
    \foreach \name / \y in {1,...,4}
        {\ifnum \y=3
            \node (O-\name) at (4*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * 0.5) {$\vdots$};
            % \node[input neuron] (I-\name) at (0,-\y-0.4) {$y_{\y}$};
        \else
            \ifnum \y=4
                \node[input neuron] (O-\name) at (4*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * 0.5) {$y_{n}^*$};
            \else
                \node[input neuron] (O-\name) at (4*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * 0.5) {$y_{\y}^*$};
            \fi
        \fi}
        
    % Forward map
    \node[Forward map] (FM) at (9*\layersep,-\nodeinlayersep * 3.) {$\mathcal{G}$};
    
    % Predicted observations 
    \foreach \name / \y in {1,...,4}
        {\ifnum \y=3
            \node (obs_p-\name) at (10*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * 0.5) {$\vdots$};
        \else
            \ifnum \y=4
                \node[input neuron] (obs_p-\name) at (10*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * .5) {$y_{n}^{**}$};
            \else
                \node[input neuron] (obs_p-\name) at (10*\layersep,-\nodeinlayersep *\y - \nodeinlayersep * .5) {$y_{\y}^{**}$};
            \fi
        \fi}    
    
    % Predicted observations - Decoder
    \foreach \name / \y in {1,...,4}
        {\ifnum \y=3
            \node (obs_p-\name) at (8*\layersep,-\nodeinlayersep *\y + \nodeinlayersep * -.5) {$\vdots$};
        \else
            \ifnum \y=4
                \node[input neuron] (obs_p2-\name) at (8*\layersep,-\nodeinlayersep *\y + \nodeinlayersep * -.5 ) {$u_{m}^{*}$};
            \else
                \node[input neuron] (obs_p2-\name) at (8*\layersep,-\nodeinlayersep *\y + \nodeinlayersep * -.5) {$u_{\y}^{*}$};
            \fi
        \fi}    
        
    % Set number of Encoder hidden layers
    \newcommand \Nhidden{3}
    % Draw Encoder 
    \foreach \N in {1,...,\Nhidden} {
        \foreach \y in {1,...,5} { %%% MODIFIED (1,...,12 -> 1,...,5, and the next five lines)
            \ifnum \y=4
                \node at (\N*\layersep,-\y*\nodeinlayersep) {$\vdots$};
            \else
                \node[hidden neuron] (H\N-\y) at (\N*\layersep,-\y*\nodeinlayersep ) {$\sigma$};
        \fi
      }
    }    
    
    % Draw Decoder
    \foreach \N in {1,...,\Nhidden} {
        \foreach \y in {1,...,5} { %%% MODIFIED (1,...,12 -> 1,...,5, and the next five lines)
            \ifnum \y=4
                \node at (\N*\layersep + 4*\layersep,-\y*\nodeinlayersep - 0*\nodeinlayersep) {$\vdots$};
            \else
                \node[hidden neuron] (D\N-\y) at (\N*\layersep + 4*\layersep ,-\y*\nodeinlayersep + 0*\nodeinlayersep) {$\sigma$};
        \fi
      }
    }        
        
    
    
    %%% <-- MODIFIED (from H\Nhidden-6 to H\Nhidden-3) 
    % Connect every node in Inputs to Encoder
    \foreach \source in {1,2,4}
        \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \draw[edge] (I-\source) -- (H1-\dest);
    
    % connect all Encoder
    \foreach [remember=\N as \lastN (initially 1)] \N in {2,...,\Nhidden}
      \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
          \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
              \draw[edge] (H\lastN-\source) -- (H\N-\dest);
              
    % Connect every node in the Encoder to output
    \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
        \foreach \dest in {1,2,4}
            \draw[edge] (H\Nhidden-\source) -- (O-\dest);
    
    % Connect to the forward operator
    \foreach \source in {1,2,4}
        \draw[edge] (obs_p2-\source) -- (FM);
        
    % Connect to the forward operator
    \foreach \source in {1,2,4}
        \draw[edge] (FM) -- (obs_p-\source);    
    
    % Connect every node in the observed output to Decoder
    \foreach \source in {1,2,4}
        \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
            \draw[edge] (O-\source) -- (D1-\dest);
            
    % connect all Decoder 
    \foreach [remember=\N as \lastN (initially 1)] \N in {2,...,\Nhidden}
      \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
          \foreach \dest in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
              \draw[edge] (D\lastN-\source) -- (D\N-\dest);
    
    
    % Connect every node in the Decoder to output
    \foreach \source in {1,...,3,5} %%% <-- MODIFIED (1,...,12 -> 1...,3,5)
        \foreach \dest in {1,2,4}
            \draw[edge] (D\Nhidden-\source) -- (obs_p2-\dest);
    
    
           
    % Pink Loss term
    \node[rectangle,fill=pink!40,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (L_misfit) at (7*\layersep, -6.6*\nodeinlayersep) {Loss $\mathcal{L}:= \halfv{\beta} \nor{\yb - \yb^*}^2 + \half \nor{\ub - \ub^*}^2 + \halfv{\alpha} \nor{\yb - \yb^{**}}^2$};
    
    % From predicted parameter to Loss term
    \draw [decorate, decoration = {calligraphic brace,mirror}, thick] (3.85*\layersep,-4.9*\nodeinlayersep) -- (4.15*\layersep,-4.9*\nodeinlayersep);
    \draw[edge,thin] (4*\layersep,-5.1*\nodeinlayersep) -- (4*\layersep, -6.1*\nodeinlayersep);
    % -- (L_misfit);

    % From predicted obs to Loss term
    \draw [decorate, decoration = {calligraphic brace,mirror}, thick] (7.85*\layersep,-4.9*\nodeinlayersep) -- (8.15*\layersep,-4.9*\nodeinlayersep);
    \draw[edge,thin] (8*\layersep,-5.1*\nodeinlayersep) -- (8*\layersep, -6.1*\nodeinlayersep);
    % -- (6.50*\layersep, -6.4*\nodeinlayersep);
    
    % From predicted obs to Loss term
    \draw [decorate, decoration = {calligraphic brace,mirror}, thick] (9.85*\layersep,-4.9*\nodeinlayersep) -- (10.15*\layersep,-4.9*\nodeinlayersep);
    \draw[edge,thin] (10*\layersep,-5.1*\nodeinlayersep) -- (10*\layersep, -6.1*\nodeinlayersep);
    % -- (6.50*\layersep, -6.6*\nodeinlayersep);
    
    
    % bracket for deep neural network
    \draw [decorate, decoration = {calligraphic brace}, thick] (.85*\layersep,-0.7*\nodeinlayersep) -- (3.15*\layersep,-.7*\nodeinlayersep) node[pos=0.5,above=0.1cm,black]{Encoder};
    
    \draw [decorate, decoration = {calligraphic brace}, thick] (4.85*\layersep,-0.7*\nodeinlayersep) -- (7.15*\layersep,-.7*\nodeinlayersep) node[pos=0.5,above=0.1cm,black]{Decoder};
    
    \draw [decorate, decoration = {calligraphic brace}, thick] (7.85*\layersep,-0.7*\nodeinlayersep) -- (10.15*\layersep,-.7*\nodeinlayersep) node[pos=0.5,above=0.1cm,black]{Model-constrained};
    
\end{tikzpicture}
\caption{Model-constrained Decoder (\mcDEC{}) deep neural network architecture. The PoI $\ub$ is fed into the encoder $\Psi_e$. The observation $\yb^*$ predicted by the encoder is fed back to the decoder  $\Psi_d$ to generate PoI $\ub^*$, which is then pushed through the PtO map $\F$ to  generate the another predicted observations $\yb^{**}$. Both predicted parameters and two observation sets are compared with ground truth $\ub$ and $\yb$, respectively, to provide the mean-square error in the loss function $\mc{L}$.}
\figlab{mcDEC_architecture}
\end{figure}



